An Energy-based Model for Word-level AutoCompletion in Computer-aided Translation

Word-level AutoCompletion(WLAC) is a rewarding yet challenging task in Computer-aided Translation. Existing work addresses this task through a classification model based on a neural network that maps the hidden vector of the input context into its corresponding label (i.e., the candidate target word is treated as a label). Since the context hidden vector itself does not take the label into account and it is projected to the label through a linear classifier, the model can not sufficiently leverage valuable information from the source sentence as verified in our experiments, which eventually hinders its overall performance. To alleviate this issue, this work proposes an energy-based model for WLAC, which enables the context hidden vector to capture crucial information from the source sentence. Unfortunately, training and inference suffer from efficiency and effectiveness challenges, thereby we employ three simple yet effective strategies to put our model into practice. Experiments on four standard benchmarks demonstrate that our reranking-based approach achieves substantial improvements (about 6.07%) over the previous state-of-the-art model. Further analyses show that each strategy of our approach contributes to the final performance.

==> sections/limitations.tex <==
\section{Limitations}

==> tables/case_study.tex <==
% % On the Language Coverage Bias for Neural Machine Translation
% \begin{table*}[t]
% \setlength{\tabcolsep}{5pt}
% \centering
% \begin{tabular}{ll cc cc cc cc}
% \toprule
% \multirow{2}{*}{\bf \#} & \multirow{2}{*}{\bf Systems}  &   \multicolumn{4}{c}{\bf Zh$\Rightarrow$En}   & \multicolumn{4}{c}{\bf De$\Rightarrow$En} \\
% \cmidrule(lr){3-6}\cmidrule(lr){7-10}
% & & \multicolumn{1}{c}{\bf Case 1}  & \multicolumn{1}{c}{\bf Case 2} & \multicolumn{1}{c}{\bf Case 3}  & \multicolumn{1}{c}{\bf Case 4} & \multicolumn{1}{c}{\bf Case 1}  & \multicolumn{1}{c}{\bf Case 2} & \multicolumn{1}{c}{\bf Case 3}  & \multicolumn{1}{c}{\bf Case 4} \\
% \midrule
% 1 & \textsc{\pb$^*$} & 1.03 & 6.04 & 3.42 & 21.30 & 3.50 & 3.83 & 2.05 & 24.47 \\
% 2 & \textsc{Ours} & 1.03 & 3.53 & 1.03 & 17.65 & 3.50 & 2.29 & 0.84 & 22.82 \\
% \bottomrule
% \end{tabular}
% \caption{The main results of our Ensemble Models and selected baselines. The results in this table are the average accuracy across four translation context types. ‘$^*$’: results are reproduced by ourselves. The best and the second-best results are in \textbf{bold} and \underline{underlined} fonts, respectively.}
% \label{tab:case_study}
% \end{table*}

% On the Language Coverage Bias for Neural Machine Translation
% \begin{table}[t]
% \setlength{\tabcolsep}{4.5pt}
% \centering
% \begin{tabular}{l cc cc}
% \toprule
% \multirow{1}{*}{\bf Systems}  &  \multicolumn{1}{c}{\bf Case 1}  & \multicolumn{1}{c}{\bf Case 2} & \multicolumn{1}{c}{\bf Case 3}  & \multicolumn{1}{c}{\bf Case 4}    \\
% \midrule
% \multicolumn{5}{c}{\it{Bi-context}}  \\
% \midrule
% \textsc{\pb$^*$} & 1.03 & 6.04 & 3.42 & 21.30 \\
% \textsc{Ours} & 1.03 & 3.53 & 1.03 & 17.65\\
% \midrule
% \multicolumn{5}{c}{\it{Prefix}}  \\
% \midrule
% \textsc{\pb$^*$} & 1.48 & 10.25 & 2.28 & 27.68 \\
% \textsc{Ours} & 1.48 & 7.40 & 1.25 & 21.18 \\
% \midrule
% \multicolumn{5}{c}{\it{Suffix}}  \\
% \midrule
% \textsc{\pb$^*$} & 1.82 & 11.05 & 2.16 & 21.87 \\
% \textsc{Ours} & 1.82 & 8.88 & 1.14 & 17.54 \\
% \midrule
% \multicolumn{5}{c}{\it{Zero-context}}  \\
% \midrule
% \textsc{\pb$^*$} & 1.59 & 15.95 & 0.00 & 28.36 \\
% \textsc{Ours} & 1.59 & 10.71 & 0.00 & 21.30 \\
% \bottomrule
% \end{tabular}
% \caption{The main results of different baselines on Zh$\Rightarrow$En Dataset. The results in this table are the average accuracy across four translation context types. ‘$^*$’: results are reproduced by ourselves. The best and the second-best results are in \textbf{bold} and \underline{underlined} fonts, respectively.}
% \label{tab:case_study}
% \end{table}

\begin{table}
    \renewcommand{\arraystretch}{1.1}
    \centering
    \small
    \begin{tabularx}{\linewidth}{|X|}
        \hline
        \multicolumn{1}{|c|}{\textbf{Case 1}}\\
        \hline
        \textbf{Source} \\
        \begin{CJK}{UTF8}{gbsn}{就膝盖而言,他说至少比手术前好了百分之百。(55)}%
        \end{CJK}\\
        \hline
        \textbf{Target Context (Zero-context)} \\
        \textcolor{blue}{le}\\
        \hline
        \textbf{\boldsymbol{$P_b$}}: \textcolor{blue}{left} \xmark \\
        \hline
        \textbf{\textsc{Ours}}: \textcolor{blue}{least} \cmark\\
        \hline
        \hline
        \hline
        \multicolumn{1}{|c|}{\textbf{Case 2}}\\
        \hline
        \textbf{Source} \\
        \begin{CJK}{UTF8}{gbsn}{计算机犯罪使美国去年损失数十亿美元(300)}%
        \end{CJK}\\
        \hline
        \textbf{Target Context (Bi-context)} \\
        computer-related crimes \textcolor{blue}{co} billions of dollars last year\\
        \hline
        \textbf{\boldsymbol{$P_b$}}: \textcolor{blue}{computer} \xmark \\
        \hline
        \textbf{\textsc{Ours}}: \textcolor{blue}{cost} \cmark \\
        \hline
        \hline
        \hline
        \multicolumn{1}{|c|}{\textbf{Case 3}}\\
        \hline
        \textbf{Source} \\
        \begin{CJK}{UTF8}{gbsn}{机场和航空公司继九一一事件后已加强了保安措施,当局这才决定减少或停止空中巡逻。(757)}%
        \end{CJK}\\
        \hline
        \textbf{Target Context (Prefix)} \\
        as airports and airlines have heightened the security since the sept.11 attacks, the \textcolor{blue}{d}\\
        \hline
        \textbf{\boldsymbol{$P_b$}}: \textcolor{blue}{decisive} \xmark \\
        \hline
        \textbf{\textsc{Ours}}: \textcolor{blue}{decided} \cmark\\
        \hline
        \hline
        \hline
        \multicolumn{1}{|c|}{\textbf{Case 4}}\\
        \hline
        \textbf{Source} \\
        \begin{CJK}{UTF8}{gbsn}{该报还指出,“如果美国继续不考虑中东国家的利益,它也将失去在海湾地区的利益。”(688)}%
        \end{CJK}\\
        \hline
        \textbf{Target Context (Suffix)} \\
        \textcolor{blue}{nat} gulf region." \\
        \hline
        \textbf{\boldsymbol{$P_b$}}: \textcolor{blue}{national} \xmark \\
        \hline
        \textbf{\textsc{Ours}}: \textcolor{blue}{nations} \cmark\\
        \hline
    \end{tabularx}
    \caption{Case study of \pb \ and \textsc{Ours} in Zh$\Rightarrow$En validation set.
    \textcolor{blue}{Text in blue} denotes the human typed characters or the predicted words.
    }
    \label{tab:casestudy}
\end{table}

==> tables/detailed_results.tex <==
% \begin{table*}[t]
%   \resizebox{2.08\columnwidth}{!}{
% \begin{tabular}{ll ccccc ccccc}
% \toprule
%   \multirow{2}{*}{\textbf{\#}} &    \multirow{2}{*}{\textbf{Systems}}         & \multicolumn{5}{c}{\textbf{De$\Rightarrow$En}} & \multicolumn{5}{c}{\textbf{En$\Rightarrow$De}} \\ \cmidrule(lr){3-7}\cmidrule(lr){8-12}
%  &            & \multicolumn{1}{l}{\textbf{Prefix}} & \multicolumn{1}{c}{\textbf{Suffix}} & \multicolumn{1}{c}{\textbf{Zero}} & \multicolumn{1}{c}{\textbf{Bi}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{Prefix}} & \multicolumn{1}{c}{\textbf{Suffix}} & \multicolumn{1}{c}{\textbf{Zero}} & \multicolumn{1}{c}{\textbf{Bi}} & \multicolumn{1}{c}{\textbf{Avg.}} \\\midrule
%     1 & \textsc{WPM-Sep*} & 57.65 & 61.46 & 50.83 & 66.15 & 59.03 & 60.48 & \underline{62.41} & 52.85 & \underline{67.08} & \underline{60.71} \\
%     2 & \textsc{Ours} & \textbf{68.69} & \textbf{70.62} & \textbf{66.40} & \textbf{76.77} & \textbf{70.62} & \textbf{69.02} & \textbf{69.25} & \textbf{60.02} & \textbf{71.87} & \textbf{67.54} \\ \bottomrule
% \end{tabular}
% }
% \caption{\label{tab:detailed} The detailed results of different systems on NIST02. We evaluate the performances of those systems on both Zh$\Rightarrow$En and En$\Rightarrow$Zh by accuracy. ‘*’: results are reproduced by ourself. The best and second-best results are in bold and underlined fonts respectively. \textcolor{red}{Prefix represents what} }
% \end{table*}

==> tables/ensemble_of_generator_and_reranker.tex <==
% On the Language Coverage Bias for Neural Machine Translation
\begin{table*}[t]
\setlength{\tabcolsep}{5pt}
\centering
\begin{tabular}{ll cc cc cc cc}
\toprule
\multirow{2}{*}{\bf \#} & \multirow{2}{*}{\bf Systems}  &   \multicolumn{2}{c}{\bf Zh$\Rightarrow$En}  & \multicolumn{2}{c}{\bf En$\Rightarrow$Zh} & \multicolumn{2}{c}{\bf De$\Rightarrow$En} & \multicolumn{2}{c}{\bf En$\Rightarrow$De}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
& & \multicolumn{1}{c}{\bf NIST05}  & \multicolumn{1}{c}{\bf NIST06} & \multicolumn{1}{c}{\bf NIST05}  & \multicolumn{1}{c}{\bf NIST06} & \multicolumn{1}{c}{\bf NT13}  & \multicolumn{1}{c}{\bf NT14} & \multicolumn{1}{c}{\bf NT13}  & \multicolumn{1}{c}{\bf NT14} \\
\midrule
% 1 &  \textsc{\pb-Sep}    & 54.15                      & 55.04                      & 53.30                      & 53.67                      &        56.93     &     55.67       &      54.54       &    51.46        \\
% 1 & \textsc{\pb} & 55.54                      & 55.85                      & 53.64                     & 54.25                             &       57.84     &    56.75   &    56.91     &      52.68      \\
1 & \textsc{\pb} & 55.52 & 56.57 & 53.90 & 54.24 & 59.11 & 56.99 & 56.89 & 53.80 \\
2 & \textsc{Ours} & \textbf{65.61} & \textbf{65.43} & \underline{60.43} & \underline{61.25} & \textbf{64.62} & \textbf{63.13} & \textbf{62.23} & \textbf{60.24} \\
3 & \textsc{Ensemble-\#1\&\#2} & \underline{64.95} & \underline{65.11} & \textbf{60.58} & \textbf{61.56} & \underline{64.21} & \underline{62.67} & \underline{61.96} & \underline{59.84} \\ 
4 & \textsc{Ensemble-\#1\&\#1$^{\prime}$} & 57.46 & 58.30 & 55.85 & 56.07 & 59.55 & 58.23 & 57.52 & 54.95 \\ 
\bottomrule
\end{tabular}
\caption{The main results of our ensemble models and selected single models on Zh$\Leftrightarrow$En and De$\Leftrightarrow$En datasets. The results in this table are the average accuracy across four translation context types.}
\label{tab:ensemble_of_generator_and_reranker}
\end{table*}

==> tables/varying_the_size_of_generator.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{l rrrr}
\toprule
\bf{System} & \bf{NIST02} & \bf{NIST05} & \bf{NIST06} & \bf{\#Para.} \\
\midrule
\textsc{\pb} & 60.93 & 55.55 &  56.27 & 100M \\ %100,459,520
\textsc{\pb-Big} & 62.27 & 56.08 & 56.97 & 288M \\ %288,999,424
\textsc{Ours} & \bf 70.12 & \bf 65.61 & \bf 65.44  & 201M \\ %201,182,209
\bottomrule
\end{tabular}
\caption{
The results of \textsc{\pb}, \textsc{\pb-Big} and \textsc{Ours} on Zh$\Rightarrow$En. The results in this
table are the average accuracy across four translation context types.
}
\label{tab:varying_the_size_of_generator}
\end{table}
